Optimal Approximate Sampling from Discrete Probability Distributions

This paper addresses a fundamental problem in random variate generation: given access to a random source that emits a stream of independent fair bits, what is the most accurate and entropy-efficient algorithm for sampling from a discrete probability distribution $(p_1, \dots, p_n)$, where the probabilities of the output distribution $(\hat{p}_1, \dots, \hat{p}_n)$ of the sampling algorithm must be specified using at most $k$ bits of precision? We present a theoretical framework for formulating this problem and provide new techniques for finding sampling algorithms that are optimal both statistically (in the sense of sampling accuracy) and information-theoretically (in the sense of entropy consumption). We leverage these results to build a system that, for a broad family of measures of statistical accuracy, delivers a sampling algorithm whose expected entropy usage is minimal among those that induce the same distribution (i.e., is "entropy-optimal") and whose output distribution $(\hat{p}_1, \dots, \hat{p}_n)$ is a closest approximation to the target distribution $(p_1, \dots, p_n)$ among all entropy-optimal sampling algorithms that operate within the specified $k$-bit precision. This optimal approximate sampler is also a closer approximation than any (possibly entropy-suboptimal) sampler that consumes a bounded amount of entropy with the specified precision, a class which includes floating-point implementations of inversion sampling and related methods found in many software libraries. We evaluate the accuracy, entropy consumption, precision requirements, and wall-clock runtime of our optimal approximate sampling algorithms on a broad set of distributions, demonstrating the ways that they are superior to existing approximate samplers and establishing that they often consume significantly fewer resources than are needed by exact samplers.

==> Makefile <==
.PHONY:all
all: clean paper arxiv

.PHONY:paper
paper:
	latexmk -pdf paper.tex

.PHONY:arxiv
arxiv: paper
	rm -rf arxiv.tar.gz
	tar cvz abstract.sh \
		appxa.tex \
		appxb.tex \
		abstract.tex \
		ACM-Reference-Format.bst \
		acmart.cls \
		assets/* \
		conclusion.tex \
		css-xml.sh \
		ddg.tex \
		experiments.tex \
		figures/* \
		fixed.tex \
		introduction.tex \
		Makefile \
		models.tex \
		optimal.tex \
		paper.bbl \
		paper.bib \
		paper.tex \
		preamble.tex > arxiv.tar.gz

.PHONY:clean
clean:
	latexmk -C *.tex
	rm -f *.aux *.bbl *.blg *.log *.dvi *.out *.idx *.bak *.toc *.lof *.fdb_latexmk
	rm -f paper.pdf paper.bbl paper.pdf arxiv.tar.gz

